scb-mt-en-th-2020: A Large English-Thai Parallel Corpus

The primary objective of our work is to build a large-scale English-Thai dataset for machine translation. We construct an English-Thai machine translation dataset with over 1 million segment pairs, curated from various sources, namely news, Wikipedia articles, SMS messages, task-based dialogs, web-crawled data and government documents. Methodology for gathering data, building parallel texts and removing noisy sentence pairs are presented in a reproducible manner. We train machine translation models based on this dataset. Our models' performance are comparable to that of Google Translation API (as of May 2020) for Thai-English and outperform Google when the Open Parallel Corpus (OPUS) is included in the training data for both Thai-English and English-Thai translation. The dataset, pre-trained models, and source code to reproduce our work are available for public use.

==> sections/related_work.tex <==
% \section{Related works}

% % 1. FACEBOOK FloRes
% % \cite{facebook_low_res}

% % 2. IWSLT 2015 TED en-th
% % https://sites.google.com/site/iwsltevaluation2015/mt-track
% % http://workshop2015.iwslt.org/downloads/proceeding.pdf

